LiFi: Lightweight Controlled Text Generation with Fine-Grained Control Codes

In the rapidly evolving field of text generation, the demand for more precise control mechanisms has become increasingly apparent. To address this need, we present a novel methodology, LIFI, which offers a lightweight approach with fine-grained control for controlled text generation. Unlike previous studies that train pre-trained language models to follow discrete, categorical, and exclusive control codes, LIFI learns controlled text generation under the guidance of continuous, relative, and nonexclusive control codes. These fine-grained codes are automatically derived from an attribute classifier, initially trained with a small amount of labeled data and subsequently employed to label abundant unlabeled data, thus garnering more extensive supervision signals. Moreover, to achieve efficient control, we incorporate the fine-grained control codes with adapters, a parameter- and compute-efficient way to steer a pre-trained language model. We evaluate LIFI on two conventional tasks -- sentiment control and topic control -- and one newly proposed task -- stylistic novel writing. Comprehensive experimental results validate the effectiveness of our proposed methods, demonstrating substantial performance improvements over existing baselines.

==> tables/tabel-human-significance-tests.tex <==
% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{cccc}
% \toprule[1pt]
% \textbf{Task} & \textbf{Baseline Model} & \textbf{Control Strength}(\%) & \textbf{Fluency} \\
% \midrule[1pt]
% Sentiment & CAT-PAW & 7.05e-7 & 3.20e-1 \\
% Topic & Fudge & 8.87e-7 & 1.65e-15 \\
% Novel & DExperts & 8.86e-9 & 7.32e-6 \\
% \bottomrule[1pt]
% \vspace{1pt} \vspace{1pt} \end{tabular}
% %}
% \caption{Significance test results on human evaluation.}
% \label{human_significance_tests}
% \end{table}

% <table>
% <tr>
%   <td>Task</td>
%   <td>Baseline Model</td>
%   <td>Control Strength</td>
%   <td>Fluency</td>
% </tr>
% <tr>
%   <td>Sentiment</td>
%   <td>CAT-PAW</td>
%   <td>7.05e-7</td>
%   <td>3.20e-1</td>
% </tr>
% <tr>
%   <td>Topic</td>
%   <td>Fudge</td>
%   <td>8.87e-7</td>
%   <td>1.65e-15</td>
% </tr>
% <tr>
%   <td>Novel</td>
%   <td>DExperts</td>
%   <td>8.86e-9</td>
%   <td>7.32e-6</td>
% </tr>
% </table>


==> tables/table-human-evaluation.tex <==
% \begin{table}[t]
% \small
% \centering
% \begin{tabular}{clcc}
% \toprule[1pt]
% \textbf{Task} & \textbf{Model} & \textbf{Win Rate}(\%) & \textbf{Fluency} \\
% \midrule[1pt]
% \multirow{2}{*}{Sentiment} & CAT-PAW & 21 & 2.51 \\
%  & \ours & \textbf{66} & \textbf{2.54}$\dagger$ \\ \midrule[0.5pt] 
% \multirow{2}{*}{Topic} & Fudge & 19 & 2.26 \\
%  & \ours &  \textbf{62} & \textbf{2.77} \\ \midrule[0.5pt] 
% \multirow{2}{*}{Novel} & DExperts & 16 & 2.26 \\
%  & \ours & \textbf{69} & \textbf{2.54} \\
% \bottomrule[1pt]
% \vspace{1pt} \vspace{1pt} \end{tabular}
% %}
% \caption{Human evaluation results. Sign tests on human scores show that our method is significantly better
% than all other methods with $p$-value $<0.01$ with the only exception marked by $\dagger$.}
% \label{human_evaluation_result}
% \end{table}
